Fairness-Aware Hybrid Precoding for mmWave NOMA Unicast/Multicast Transmissions in Industrial IoT

This paper investigates dual-layer non-orthogonally superimposed transmissions for industrial internet of things (IoT) millimeter-wave communications. Essentially, the overlayer is a ubiquitous multicast signal devised to serve all the devices in coverage with a common message, i.e., critical control packet. The underlayer is a composite signal that consists of private unicast messages. Due to safety implications, it is critical that all devices can decode the multicast information. To ensure this requirement, we jointly optimize the hybrid precoder, analog combiners, power allocation, and fairness. Specifically, we incorporate a power splitting constraint between the two overlaid signals and enforce supplementary per-device constraints to guarantee multicast fairness. Performance is evaluated in terms of the spectral efficiency, multicast fairness, and bit error rate, thus corroborating the feasibility of our proposed scheme.

==> text/overview.tex <==
\section{Overview}
\label{sec:overview}

\subsection{Contribution}
\begin{enumerate}
\item Determine the optimal power ratio for coexisting unicast and multicast transmissions in both time and frequency domain. 
\item The existing multicast grouping technique solely for multicast transmission without underlying unicast transmission is suboptimal because: $(i)$ given that nodes are within the a close proximity of one another, serving them simultaneously induces high interference, and thus they must not be scheduled within the same time period.     
\end{enumerate}



\subsection{Ongoing work}

\subsubsection{PHY layer optimization}
We aim to optimize for power ratio to achieve one/more of the following goals: 
\begin{itemize}
\item Fairness
\item Throughput
\item Delay
\item SINR
\end{itemize}

\subsubsection{MAC layer optimization}
We propose a scheduling algorithm to optimize the multicast and unicast grouping in order to determine the subset of nodes that should be served together. The schedule might be incorporated into the formulation of the PHY layer optimization. 



\subsection{Potential challenge}
\begin{enumerate}
\item Incorporating nodes grouping within the optimization for power ratio. 
\item In dense scenarios, when all the nodes are clustered within the same area, the best one can do is to transmit unicast/multicast sequentially, i.e., the number of transmission $=$ number of nodes.   
\end{enumerate}



\subsection{Tentative/Future plan}
\begin{enumerate}
\item Adapting power ratio such that the transmission time for both multicast and unicast transmission is minimized and synchronized. 
\item The assumption of NOMA that there is no notion of time-slot since all users are served simultaneously is non-beneficial when the unicast user are having highly correlated channel, or when the multicast rate is too low \cite{riazul:2017:noma}. Therefor executing such transmission with multiple time-slot is better. 
\item Developing low-complexity resource allocation algorithms is important, as they play a pivotal role for NOMA performance optimization \cite{riazul:2017:noma}. User pairing and power allocation have been considered. 
\end{enumerate}

==> text/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
